PRAGO: Differentiable Multi-View Pose Optimization From Objectness Detections

Robustly estimating camera poses from a set of images is a fundamental task which remains challenging for differentiable methods, especially in the case of small and sparse camera pose graphs. To overcome this challenge, we propose Pose-refined Rotation Averaging Graph Optimization (PRAGO). From a set of objectness detections on unordered images, our method reconstructs the rotational pose, and in turn, the absolute pose, in a differentiable manner benefiting from the optimization of a sequence of geometrical tasks. We show how our objectness pose-refinement module in PRAGO is able to refine the inherent ambiguities in pairwise relative pose estimation without removing edges and avoiding making early decisions on the viability of graph edges. PRAGO then refines the absolute rotations through iterative graph construction, reweighting the graph edges to compute the final rotational pose, which can be converted into absolute poses using translation averaging. We show that PRAGO is able to outperform non-differentiable solvers on small and sparse scenes extracted from 7-Scenes achieving a relative improvement of 21% for rotations while achieving similar translation estimates.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% Background on Pose Estimation
The estimation of a set of camera poses given the corresponding images is an important problem within Computer Vision, which lies at the heart of Structure-from-Motion (SfM) pipelines. However, with the current abundance of images and increasing availability of computational resources, most approaches focus on optimization with assumptions of large and dense camera pose graphs, with relatively short baselines or expendable images. The SfM estimation absolute camera poses is a well-established pipeline using matched keypoints between images~\cite{snavelySIGGRAPH06photo}.
Where initial relative poses can be estimated by 5 or 8 Point algorithms. 
From such initial relative poses, absolute pose can be inferred by the combination of rotation averaging~\cite{9577752,Lee_2021_CVPR,purkait2020neurora} and translation averaging~\cite{990963,zyesil2014RobustCL,snavely_translationavg} or the combined motion averaging~\cite{arrigoni2016spectral}. 





% Benefits of Pose Refinement including objectness
Approaches for SfM are robust on large collections where they can apply outlier rejection on the input~\cite{wilson_eccv2014_1dsfm} or as internal step~\cite{purkait2020neurora}. Alternatively, recently the use of objectness-based detections has been shown as a way to refine relative poses (PoserNet~\cite{taiana2022posernet}), by reasoning on this higher-level semantic information without the removal of edges. The authors proposed a novel graph-based approach incorporating the detections on the image nodes of the graph, and the aggregate of predictions of the refined relative pose on the edges. Message passing propagated information in an MLP-style alternating updates between nodes and edges. While showing an improvement, the approach remained disconnected from the remaining pipeline. 

Similarly, in rotation averaging, there have been numerous efforts to develop differentiable rotation averaging based on an input relative pose graph. Recent methods such as NeuRoRA~\cite{purkait2020neurora}, optimize the rotational elements of the pose graph firstly filtering the graph and then inferring the rotations. Alternatively, RAGO proposed an optimization-based differentiable approach with multiple steps of inference of the graph construction. With the pose aforementioned outlier, small graphs pose a significant challenge to these methods, while remaining detached from prior steps.

In contrast, we propose PRAGO, a differentiable pose estimatiomn method,  which focuses on small and sparse pose graphs where outlier rejection would be unsuitable while taking advantage of higher-level information such as objectness detections. PRAGO utilizes an objectness based approach to camera pose refinement and integrates it with rotational averaging, we show that optimizing these tasks together can create a significant improvement. While PRAGO does not make decisions early on the viability of the pose graph, which makes it highly suitable for small and sparse graphs. To understand the effect we provide an analysis of the orientation error and identify that frequent chirality errors are fixed through the PRAGO model. As well as comparisons to state-of-the-art combinations of independent methods both differentiable or optimization.  

We make three major contributions: 
\emph{1)} introduce the PRAGO network for differentiable pose estimation with objectness detections where the back-propagation improves performance in contrast to non-differential pipelines;
\emph{2)} revise the objectness pose refinement ~\cite{taiana2022posernet} which leads to improved accuracy;
and \emph{3)} An analysis of how objectness-based pose refinement improves relative poses and its positive effect on chirality even when combined with other components. 

%\NETNAMEwithSpace an enhanced  version of~\cite{taiana2022posernet} which leads to improved accuracy; 
%\emph{2)} Fusion of \NETNAMEwithSpace and absolute pose estimation pipeline (rotation and translation averaging;
%\emph{3)} The fully-differentiable combination of  \NETNAMEwithSpace with RAGO, a differentiable rotational averaging method, which leads to a further increase in rotational averaging accuracy;   


%We incorporate such an approach into PRAGO and provide a supporting analysis that shows how objectness pose refinement is a fundamental task to overcome chirality issues when outlier rejection is not feasible or desired. 

%that have the potential to be trained in a fully-differentiable fashion together with a pose refining module, improving the overall outcome. We, therefore, evaluate the benefits of objectness-based pose refinement in combination with two State-of-The-Art methods:  and RAGO~\cite{li2022rago}. Moreover, we integrate the proposed \NETNAMEwithSpace with RAGO to form a fully differentiable pipeline, so that \NETNAMEwithSpace can benefit from the supervision signal originating with absolute orientations. This arrangement is shown to lead to an improved rotation averaging performance. 



% Differentiable Rotational Averaging
%In addition, while the PoserNet method is differentiable, it does not exploit information from the subsequent step of rotation averaging during its training. Instead, the authors rely on the {EIG-SE3} optimization approach to solve the motion averaging problem, without the possibility of gradients being propagated back to PoserNet. However, 
%There have been numerous efforts to develop differentiable rotation averaging that have the potential to be trained in a fully-differentiable fashion together with a pose refining module, improving the overall outcome. We, therefore, evaluate the benefits of objectness-based pose refinement in combination with two State-of-The-Art methods: Neurora~\cite{purkait2020neurora} and RAGO~\cite{li2022rago}. Moreover, we integrate the proposed \NETNAMEwithSpace with RAGO to form a fully differentiable pipeline, so that \NETNAMEwithSpace can benefit from the supervision signal originating with absolute orientations. This arrangement is shown to lead to an improved rotation averaging performance. 


%Such a graph structure is complex to instantiate and iterate on; therefore, we propose a simpler Edge Graph Attention Network (EGAT) formulation, which we name \NETNAME, that achieves a slight increase in pose accuracy.


%In this work, we explore the task of training the combination of a method which refines relative poses exploiting potential object region matches with a rotation averaging system in a fully differentiable way, with the goal of improving rotation averaging and motion averaging performance.    

% Background 









%Finally, in an effort to understand how pose refinement improves the performance of rotation averaging methods, we investigate the angular error change induced by \NETNAMEwithSpace and highlight that the initial chirality errors are greatly reduced by PoserNet style architecture. The effect can be compared to that achieved by algorithms designed to perform outlier rejection in the context of rotation averaging, such as CleanNet from~\cite{purkait2020neurora}, or 1DSFM~\cite{wilson_eccv2014_1dsfm}, but without the disadvantage of reducing the connectivity of the graph. This is especially important when dealing with small pose graphs when removing edges from the pose graph could strongly negatively affect the final reconstruction.

% Contributions



% \emph{3)} Providing an analysis of independent modules and their joint improvement on absolute poses; and \emph{4}, 


==> sec/4_Chirality.tex <==
\section{On the noise in relative poses}


% By Matteo Taiana, this was integrated in Related Work on relative pose estimation.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Relative pose estimates are noisy, because of how they are generated.
% The first step for estimating a set of absolute camera poses consists in estimating pairwise relative poses. If such pairwise poses were to be perfectly accurate, motion averaging would be a trivial task. The very nature of how the relative poses are computed, instead, leads to relative poses with varying degrees of error, with some error almost as large as $180^\circ$. Though many different variants exist of such pairwise pose estimation pipeline, most follow similar steps. Initially, distinctive keypoints are detected on both images of a pair. Then, keypoints are matched based on an encoding of their appearance. But appearance can vary substantially when one 3D point is imaged from very different camera poses, or at different times of the day or year (as is common in the SfM setting), making the matching error-prone. The second step in the pipeline involves estimating a relative pose supported by as much evidence as possible. Thus, methods for estimating the Essential matrix, such as the 5-point algorithm, are combined with outlier-rejection methods such as RANSAC. This, depending on the number and quality of the matched keypoints, tends to result in estimates with a low level of noise. Furthermore, computing a rotation matrix and a translation unit vector from the Essential matrix presents an inherent ambiguity, as two solutions exist for each of them~\cite{Nister, look paper up in bibliography}. One of the four solution is chosen based on chirality considerations (triangulated 3D points should be in front of both cameras). Picking one of the incorrect combinations is what can result in very large errors.
%
% % Motion averaging algorithms employ some strategies to deal with the noise.
% Motion averaging algorithms are often designed to deal with these kinds of errors. For example, NeuRoRA has an architecture based on two GNNs, the first of which (CleanNet) is tasked with removing outlier relative orientations and refining the rest of them. Similarly, the first step in 1DSfM consists in removing translation outliers. Considering that in the case of sparse pose graphs rejecting relative poses can lead to catastrophic results (a graph with multiple components does not contain enough information for estimating coherent absolute poses), we design \NETNAMEwithSpace to refine relative poses, without rejecting any of them.


% This was elaborated on in Related Work.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The purpose of including \NETNAMEwithSpace in the motion averaging pipeline is to both reduce the overall level on noise, and to identify and correct outliers with large errors due to wrong chirality~\cite{Hartley2004Chirality}. The latter is a common problem in relative pose estimation, due to the fact that given a pair of cameras with matched 2D keypoints, geometric approaches based on perspective geometry will provide two possible poses. Of these, one is the correct pose, and the other a physically impossible solution, that places the image points behind the camera and corresponds to the correct pose but with the orientation rotated by $180^\circ$. This means that, if the relative pose algorithm selects the solution with the wrong chirality, it will provide a relative pose with an error of about $180^\circ$. 

Classical approaches usually address this by identifying the outliers measurements by imposing cycle consistency, \ie chaining relative transformations along a closed loop~\cite{5539801}, which can be simplified by projecting the problem to a lower dimension~\cite{wilson_eccv2014_1dsfm}. These approaches are well suited to large graphs, with a large number of connections, that have enough cycles to allow identifying the outliers. 
In the case of the graphs used by PoserNet, however, such methods are not applicable due to the limited number of nodes, eight, and sparse connections. 


In fact, only $XX \%$ of the possible edges have an observed relative pose. Instead, we rely on a model based on PoserNet~\cite{taiana2022posernet} as a way to learn to correct relative poses with the wrong chirality. This is validated by looking at the distribution of per-edge relative orientation errors on the input and output of PoserNet, as shown in Figure~\ref{fig:chirality_reduction}. From this distribution we can see that most of the relative orientations generated by the 5 Point algorithm have errors smaller than $25^\circ$, while a small fractions - $XX \%$ - have large errors, close to $180^\circ$, \ie due affected by chirality errors. Looking at the output, we can see how on a large fraction of edges - $XX \%$  - the noise is almost zero, and the errors larger than $25^\deg$ have all been corrected. 

%The observed relative rotations given as input to rotation averaging are affected by noise and the presence of outliers. One type of outliers is due do chirality errors~\cite{Hartley2004Chirality}, that happen when the relative pose estimation algorithm finds a mathematically correct but physically impossible solution that places the image points behind the camera. This results in a camera orientation that is opposite (\ie rotated by $180^\circ$) with respect to the correct solutions. This is the case for some of the input relative poses that PoserNet~\cite{taiana2022posernet} generates from 7Scenes through the 5-point algorithm.

% This was rephrased in Related Work. 
This is usually addressed by outliers as identifying measurements that cannot be consistently chained along cycles~\cite{5539801}, which can be simplified by projecting the problem to a lower dimension~\cite{wilson_eccv2014_1dsfm}. This, however, works best when the graph is large and rich in connections; in contrast, PoserNet uses small graphs (8 nodes), whit sparse connections (only $XX \%$ of the possible edges have an observed relative pose). For this reason, we instead opt for a learning-based approach, using PoserNet~\cite{taiana2022posernet} to learn to correct relative poses with the wrong chirality.


As reported in Figure~\ref{fig:chirality_reduction}, we can see how the noise on the relative orientations provided as input to PoserNet is, in most cases, smaller than $25^\circ$. A small fraction of edges ($XX \%$ ) present noise close to $180^\circ$, which can be attributed to chirality errors in the 5point relative pose estimate. We can see how PoserNet corrects these large errors, at the cost of a small increase ($XX \%$ ) of the noise on the other edges. 

This supports the claim that an approach based on PoserNet will be able to correct the poses with the wrong chirality, which could have significant repercussion on the downstream motion averaging modules by removing sources of large noise. 

% \begin{figure*}[th!]
%         \centering
%         \begin{subfigure}{.245\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{Images/with_vs_without_PN_NeuRoRA_transparent.eps}
%             \caption{}
%         \end{subfigure}
%                 \begin{subfigure}{.245\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{Images/with_vs_without_PN_NeuRoRA_logY_transparent.eps}
%             \caption{}
%         \end{subfigure}
%         \begin{subfigure}{.245\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{Images/with_vs_without_PN_NeuRoRA_transparent.eps}
%             \caption{}
%         \end{subfigure}
%         \begin{subfigure}{.245\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{Images/with_vs_without_PN_NeuRoRA_logY_transparent.eps}
%             \caption{}
%         \end{subfigure}
%     \caption{\emph{Effect of PoserNet+ refinement on downstream tasks}: error distribution for all camera absolute orientations generated by NeuRoRa~\cite{purkait2020neurora} (a) and RAGO~\cite{li2022rago} (c) with (yellow) and without (blue) PoserNet refinement. For ease of viewing, we present the same distributions in semi-log scale (b,d respectively).}\label{fig:posernet_effect}
% \end{figure*}


==> sec/5_evaluation.tex <==
\section{Evaluation}


\begin{table*}[t]
    \scriptsize
    \centering
    \begin{tabularx}{\textwidth}{k X c c c c c c c c c c c c}
    \toprule
         &         & \multicolumn{6}{c}{Orientation error (deg)}        & \multicolumn{6}{c}{Translation error (meters)}               \\ \cmidrule(lr){3-8} \cmidrule(lr){9-14}
    Method   &  & 3 & 5 & 10 & 30 & 45 & $\eta$ & 0.05 & 0.1 & 0.25 & 0.5 & 0.75 & $\eta$ \\\midrule
    \multirow{4}{*}{EIG-SE3} 
    & w/o PoserNet   &    
         12.79  & 
         24.88  &  
         35.80  & 
         58.71  & 
         62.59  &       
         25.22  &
         
          0.00  & 
          0.06  &   
          2.70  & 
         31.70  &  
         73.99  &       
          0.61  \\
         \cmidrule(lr){3-14} 
         
     & w. PoserNet     &  
         16.09   & 
         50.44   &  
         85.43   & 
         94.44   & 
         96.30   &       
          4.97   &

          0.06   & 
          2.01   &   
         35.85   & 
 \textbf{78.38}   &  
 \textbf{94.82}   &       
         0.32    \\ \cmidrule(lr){3-14} 
         
     & w. \NETNAMEwithSpace     &  
         28.15  & 
 \textbf{60.26}  &  
         85.72  & 
         94.43  & 
         96.55  &       
  \textbf{4.21}  &
         
          0.04   & 
          2.69   &   
         34.88   & 
         76.21   &  
         94.19   &       
          0.33   \\
         
    \midrule
    \multirow{4}{*}{NeuRoRA, BATA} & w/o PoserNet      & 
         17.10  & 
         42.55  &  
         70.41  & 
         91.37  & 
         95.94  &       
          5.84  &
         
          0.18  & 
          1.20  &   
          7.16  & 
         35.27  &  
         69.51  &       
          0.61  \\  \cmidrule(lr){3-14}

         & w. \NETNAMEwithSpace     & 
         22.60  & 
         55.91  &  
         84.89  & 
         95.97  & 
         97.37  &       
          4.59  &
         
         1.20  & 
        10.07  &   
        36.89  & 
        66.68  &  
        85.77  &       
         0.35  \\ 
         
    \midrule
    \multirow{6}{*}{RAGO, BATA} & w/o PoserNet      & 
         21.60  & 
         48.95  &  
         76.08  & 
         93.17  & 
         96.29  &       
          5.09  &
         
          0.13  & 
          1.01  &   
          7.44  & 
         35.75  &  
         69.68  &       
          0.60    \\  \cmidrule(lr){3-14}
         
         & w. \NETNAMEwithSpace      & 
 \textbf{28.84}  & 
         59.68  &  
 \textbf{87.28}  & 
 \textbf{96.17}  & 
 \textbf{97.53}  &       
          4.26  &
         
 \textbf{ 1.50}   & 
 \textbf{11.59}  &   
 \textbf{40.97}  & 
         71.58   &  
         90.09  &       
 \textbf{0.31}    \\  
         
         % Double line
         \cmidrule(lr){3-14} 
         \noalign{\vskip0.5pt\doublerulesep
         \vskip-\arrayrulewidth}
         \cmidrule(lr){3-14}

        & Joint (simple loss sum) & 
         37.88  & 
         65.59  &  
 \textbf{89.29}  & 
         96.32  & 
         97.56  &       
         3.77  &
         
          0.34  & 
          4.47  &   
         33.23  & 
         67.84  &  
         89.41  &       
          0.36    \\  \cmidrule(lr){3-14}

       & Joint (weighted loss sum) & 
          35.73  & 
          64.31  &  
          88.68  & 
          96.30  & 
          97.55  &       
          3.87  &
         
 \textbf{ 1.63}  & 
 \textbf{11.66}  &   
 \textbf{40.89}  & 
 \textbf{71.79}  &  
 \textbf{90.51}  &       
 \textbf{ 0.32}  \\  \cmidrule(lr){3-14}

       & Joint (only RAGO loss) & 
 \textbf{38.37}  & 
 \textbf{66.28}  &  
          89.17  & 
 \textbf{96.36}  & 
 \textbf{97.59}  &       
 \textbf{ 3.75}  &
         
           0.00  & 
           0.00  &   
           2.90  & 
          31.09  &  
          70.14  &       
           0.61    \\ 

    \bottomrule
    \end{tabularx}
    \centering
    \caption{\label{tab:results_posernet_followed_by_x}
    Absolute pose error. To facilitate comparison, the best value for each column has been highlighted both for the method combinations that were trained in a fully differentiable way (bottom three rows) and for the ones that were not trained that way (top seven rows). Internal notes:  "Vanilla" NeuRoRA performs quite a lot better than "vanilla" EIG-SE3. This probably happens because "vanilla" NeuRoRA is actually fine-tuned on our 5pts training data.}
    % describes data used as input for PoserNet, while ``Refined'' describes its output. $\eta$ indicates median values. For both initialisation techniques, Both for BB and keypoint based input, PoserNet is effective at refining relative poses in terms of orientation and translation direction.}
\end{table*}

% 1. Intro to section.
% 2. The data: number of graphs, etc.
% 3. Analysis on how PN++ affects relative noise.
% 4. Experiment 1: effect of using PN vs OptPN with EIG-SE3. 
% 5. Experiment 2: effect of using OptPN followed by three different Motion Averaging systems: EIG-SE3, NeuRoRA followed by BATA, and RAGO followed by BATA.
% 6. Experiment 3: effect of training OptPN and RAGO separately or jointly (with ablation).

We present results obtained working on view graphs selected from the 7-scenes dataset~\cite{glocker2013real-time}. In the first experiment, we characterize the effect \NETNAMEwithSpace has on relative orientation estimates. In the second experiment, we highlight the positive impact of using the proposed \NETNAMEwithSpace rather than PoserNet in combination with EIG-SE3. The third experiment compares the motion averaging performance achieved by three different methods when working on raw pairwise relative poses versus when the relative poses have been refined by \NETNAMEwithSpace. In the last experiment, we show that \NETNAMEwithSpace can be combined with RAGO to form a fully-differentiable module, leading to an improvement in the rotation averaging performance. For all the experiments, to summarize the results we aggregate errors by computing a graph-wise mean (the mean camera orientation error for a graph) and then computing the median of such averages. 


% The reconstructed and ground-truth poses are, however, expressed in different reference systems; to compare them, we translate the reconstructions to make the center of mass of the cameras coincide, and estimate a rigid global rotation and scaling that minimizes the Euclidean distance between the two sets of poses.

\textbf{Dataset --} We use the view graphs from the ``small graphs dataset'' proposed in~\cite{taiana2022posernet}, which is based on images and camera poses from the 7-Scenes dataset. The data consists of $14000$ training graphs ($2000$ per scene) and $7000$ test graphs ($1000$ graphs per scene). Each graph contains eight nodes, with a connectivity dictated by the success of estimating a relative camera pose between the two images using SuperGlue, the five-point algorithm and RANSAC. This results in an average of $15.5$ edges per graph out of the possible $28$ edges ($55.36\%$ connectivity). In spite of what is claimed in~\cite{taiana2022posernet}, $3.8\%$ of the test graphs do not contain one single component, but multiple ones. Having a graph partitioned in separate components makes it impossible to estimate coherent absolute poses for all the cameras. To avoid this problem, we present results on the $6731$ test graphs which form one single component. \textbf{ToDo: talk about the matched detections, but defer to ECCV paper for details.}


\textbf{Refining relative poses with \NETNAMEwithSpace --} 
In~\cite{taiana2022posernet}, PoserNet was shown to succeed in refining relative poses and, thus, to lead to more accurate absolute poses. In this experiment, we characterize the effect \NETNAMEwithSpace has on estimates affected by different levels of noise. From the edge-wise orientation error histograms in Fig.~\ref{fig:chirality_reduction} it can be seen that \NETNAMEwithSpace greatly reduces the number of estimates with orientation error larger than $160^\circ$, the ones which likely stem from an incorrect chirality choice.  
The transfer matrix on the right side of Fig.~\ref{fig:chirality_reduction} visualizes the effect \NETNAMEwithSpace has on estimates affected by different levels of noise. Elements below and above the main diagonal correspond to estimates whose accuracy is increased or decreased, respectively. On the bottom-left corner of the matrix, it can be seen that many estimates with the wrong chirality are corrected to very accurate values (many of the input estimates that fall in the bin centered at $176^\circ$ are corrected to estimates that fall in the bin centered at $1^\circ$). This chirality-correction property is not perfect, though, as as other such estimates are corrected to estimates with lower, but non-negligible levels of error (e.g., estimates that are moved from the bin centered on $176^\circ$ to that centered on $46^\circ$). 
Other effects are visible on the matrix, though perhaps not as clearly or not with a straightforward interpretation. On the top-left corner of the matrix, it can be seen that estimates with lower input errors can be affected both positively and negatively by \NETNAME. Finally, the high values present on the first column of the matrix indicate that many estimates are corrected to very low error values.   

This analysis highlights that \NETNAMEwithSpace has a strong positive impact on estimates affected by incorrect chirality, while also improving other estimates, suggesting that it could be especially important when coupled with motion averaging systems which do not implement an outlier rejection strategy.


\textbf{\NETNAMEwithSpace vs PoserNet --} In this experiment, we compare the performance obtained by EIG-SE3 when being applied respectively on raw relative poses, on poses refined by PoserNet and on poses refined by the proposed \NETNAME. As can be seen in Tab.~\ref{tab:results_posernet_followed_by_x}, refining the relative poses with either version of PoserNet before processing them with EIG-SE3 leads to a large improvement in the accuracy of both rotation averaging (median error drops from $25.22^\circ$ to below $5^\circ$) and translation averaging (median error almost halves from $0.6 \:m$ to $0.3 \:m$. Applying the proposed \NETNAMEwithSpace rather than PoserNet affords a drop in median orientation error from $4.97^\circ$ to $4.21^\circ$, with the percentage of nodes with error below $3^\circ$ increasing from $16.09\%$ to $28.15\%$. The corresponding impact on median translation error is negligible. As can be seen in Fig.~\ref{fig:absolute_orientation_error_OptPoserNet_followed_by_x}~(a), EIG-SE3 is not able to solve all the chirality errors present in the raw input data (a considerable number of nodes has orientation estimates with errors close to $180^\circ$). Applying EIG-SE3 on the refined relative poses provided by \NETNAMEwithSpace leads to much more accurate absolute orientation estimates, in part because \NETNAMEwithSpace is able to resolve most of the chirality errors. 


\textbf{\NETNAMEwithSpace followed by Motion Averaging -} In this experiment, we compare the performance achieved by pairing \NETNAMEwithSpace with three different Motion Averaging systems: EIG-SE3, NeuRoRA followed by BATA, and RAGO followed by BATA. For these systems, to the extent that was possible, we relied on the code distributed by their authors\footnote{In case part of the code was missing, we implemented it according to the information contained in the respective papers.}. 
It is important to notice that EIG-SE3 is not trainable, so it is applied without any customization to the problem. For NeuRoRA, we fine-tuned the pre-trained networks (both CleanNet and FineNet) on the training data from 7-Scenes as provided in~\cite{taiana2022posernet}. We trained RAGO from scratch on the same training data and applied it on our test data directly. The authors of RAGO mention that they preprocess real data with NeuRoRA's CleanNet, but for our experiments, we opted to apply it directly on raw relative poses or to the refined relative poses produced by \NETNAME. Like EIG-SE3, BATA is not trainable, so it was applied directly as is distributed by its authors. While in~\cite{taiana2022posernet} PoserNet was also combined with MultiReg~\cite{yew2021learning} as a motion averaging module, we do not do so because MultiReg requires an input which is not usually available in SfM settings: the absolute scale of relative translations. 

\begin{table}[t]
    \scriptsize
    \centering
    \begin{tabularx}{\columnwidth}{X c c }
    
    \toprule
    
    Loss              & {Orientation error (deg)}        & {Translation error (meters)} \\
    \midrule

    Only RAGO Losses &
         3.75  & 
         0.61   \\                 
    \midrule

    Simple sum  &
         3.77  & 
         0.36    \\                 
    \midrule

    Weighted sum  &
         3.87  & 
         0.32    \\                 
    \bottomrule
    
    \end{tabularx}
    \centering
    \caption{\label{tab:loss_ablation}
    Ablation on loss combination in \NETNAMEwithSpace \& RAGO. 
    %Only RAGO leads to best orientation accuracy, but translation accuracy is quite bad. Simply adding the two losses leads to good results, weighting the losses before adding them leads to similar, but more balanced results? Translation seems better when looking at the other table, but not so much in terms of median. }
    % describes data used as input for PoserNet, while ``Refined'' describes its output. $\eta$ indicates median values. For both initialisation techniques, Both for BB and keypoint based input, PoserNet is effective at refining relative poses in terms of orientation and translation direction.
    }
\end{table}


\begin{figure*}[t]
        \centering
    \begin{tabular}{cccc}
          \includegraphics[width=39mm]{Images/with_vs_without_PN_EIG-SE3_transparent.pdf}      &  
          \includegraphics[width=39mm]{Images/with_vs_without_PN_NeuRoRA_transparent.pdf}      & 
          \includegraphics[width=39mm]{Images/with_vs_without_PN_RAGO_transparent.pdf}         &
          \includegraphics[width=39mm]{Images/joint_PN_and_RAGO_transparent.pdf} \\

          \includegraphics[width=39mm]{Images/with_vs_without_PN_EIG-SE3_logY_transparent.pdf}      &  
          \includegraphics[width=39mm]{Images/with_vs_without_PN_NeuRoRA_logY_transparent.pdf} & 
          \includegraphics[width=39mm]{Images/with_vs_without_PN_RAGO_logY_transparent.pdf}    &
          \includegraphics[width=39mm]{Images/joint_PN_and_RAGO_logY_transparent.pdf}          \\
          
          \small (a) EIG-SE3 & (b) NeuRoRA &  (c) RAGO & (d) Joint PN, RAGO\\
    \end{tabular}
    \caption{ Absolute orientation error of \NETNAMEwithSpace followed by different motion averaging methods. (The Joint PN+RAGO column refers to the SIMPLE SUM version).
    }\label{fig:absolute_orientation_error_OptPoserNet_followed_by_x}
\end{figure*}

\begin{figure}
        \centering
    \begin{tabular}{c}
          \includegraphics[width=0.49\linewidth]{Images/joint_vs_separated_PN_and_RAGO_transparent.pdf}     
          \includegraphics[width=0.49\linewidth]{Images/joint_vs_separated_PN_and_RAGO_logY_transparent.pdf}   
    \end{tabular}
    \caption{ Effect of training \NETNAMEwithSpace and RAGO separately or in a fully differentiable way. Training the two modules together has a largely positive effect on the estimates of absolute orientations.}\label
    {fig:separated_vs_joint_OptPoserNet_and_RAGO}
\end{figure}

As can be seen in Tab.~\ref{tab:results_posernet_followed_by_x} and in Fig.~\ref{fig:absolute_orientation_error_OptPoserNet_followed_by_x}, applying \NETNAMEwithSpace on the raw relative poses is beneficial for all motion averaging algorithms, with the median translation error dropping from roughly $0.6 \:m$ to roughly $0.3 \:m$ for all of them. In terms of absolute orientation errors, EIG-SE3 is the algorithm which benefits the most from the relative pose refinement. When applied on raw relative transformations, EIG-SE3 produces the estimates with the highest median rotational error ($25.22^\circ$), highlighting a sensitivity to highly noisy input data. When applied on refined relative poses, instead, EIG-SE3 produces the lowest median orientation error of all methods not trained in a fully-differentiable way with \NETNAMEwithSpace ($4.21^\circ$), narrowly beating RAGO.

\textbf{Fully differentiable VS separated \NETNAMEwithSpace and RAGO --} In this experiment, we compare the performance achieved by training \NETNAMEwithSpace and RAGO independently, with that achieved by training them as a single, fully differentiable module. When training the fully differentiable module, the problem arises of how to best combine the losses of the single components. Defining the combined loss as: $$\mathcal{L} = \alpha \cdot \mathcal{L}_{PN++} + \beta \cdot \mathcal{L}_{RAGO}$$ with $\mathcal{L}_{PN++}$ being the total loss of \NETNAMEwithSpace and $\mathcal{L}_{RAGO}$ that of RAGO, we devised three strategies: driving the learning using exclusively RAGO's loss ($\alpha = 0, \beta=1$), driving it by naively adding the two loss components ($\alpha = 1, \beta=1$) and, finally, driving the learning by weighting the loss components so that they would have comparable values at the end of the training of the single components ($\alpha = 1, \beta=0.01$). As can be seen in Tab.~\ref{tab:results_posernet_followed_by_x}, training \NETNAMEwithSpace and RAGO as a combined system leads to an improved performance in terms of rotation accuracy, and can be done without negatively affecting the accuracy on the translation. Relying exclusively on RAGO's loss leads to the overall best results in terms of rotation averaging, with a median error of $3.75^\circ$ as opposed to $4.21^\circ$ for the best non-fully-differentiable system (\NETNAMEwithSpace followed by EIG-SE3). But this results comes with a large penalty for translation averaging, with the median error raising as high as when the methods are run on raw relative pose data ($0.62 \:m)$. The other two loss combination strategies have a clear advantage respect to the first one in terms of translation averaging, with the median error roughly dropping from $0.6 \:m$ to $0.3 \:m$, while still beating all the non-fully-differentiable systems in terms of rotation error. The histogram of orientation errors obtained by applying separately trained \NETNAMEwithSpace and RAGO versus by applying the system trained in a fully differentiable way are shown in Fig.~\ref{fig:separated_vs_joint_OptPoserNet_and_RAGO}.



% \textbf{ToDo: explain this.} In the original PoserNet paper the authors evaluated against  MultiReg~\cite{yew2021learning}; we do not do this as it requires large, densely connected graphs and an estimate of the size of the tranlsations to work correclty. (3DV 2021) claims to perform Motion Averaging, but the author wrote me: ``MultiReg can only work on the motion averaging task where the absolute scales of translations are known'';









\subsection{Implementation details}
As the input relative poses, we used the five-point poses from~\cite{taiana2022posernet}. We implemented \NETNAMEwithSpace using the PyTorch framework~\cite{pytorch} and PyTorch Geometric~\cite{FeyLenssen2019pyg}, and trained it using the Adam optimizer with learning rate $0.0001$ and batch size $1$. We used a schedule to reduce the learning rate by a factor of $0.316$ with a patience of $3$ epochs. We used the author implementation for each of the other methods, EIG-SE3\cite{arrigoni2016spectral},  RAGO~\cite{li2022rago}, NeuRoRA~\cite{purkait2020neurora} and BATA~\cite{zhuang2018baseline}. For training or fine-turning those methods, we used the training set defined in~\cite{taiana2022posernet}, and the hyperparameters present in their code or defined in their papers. For the joint training of \NETNAMEwithSpace and RAGO, we started from versions of the models that had been trained in isolation, and fine-tuned the the joint system using the same hyperparameters used for \NETNAME.


==> sec/zzz_backup_5_evaluation.tex <==
\section{Evaluation}

We present results in terms of absolute rotation error and absolute translation error. 
\begin{itemize}
  \item We compare the performance afforded by PoserNet and by PoserNet v2 when combined with EIG-SE3. 
  \item We compare the performance of three motion averaging systems: EIG-SE3, NeuRoRA followed by BATA, and RAGO followed by BATA.
  \item We compare the performance of PoserNet v2 followed by RAGO when trained separately or jointly, and we ablate the performance of the joint system when trained with different weights for the loss components.
\end{itemize}



\begin{table*}[t]


    \scriptsize
    \centering
    \begin{tabularx}{\textwidth}{k X c c c c c c c c c c c c}
    \toprule
         &         & \multicolumn{6}{c}{Orientation error (deg)}        & \multicolumn{6}{c}{Translation error (meters)}               \\ \cmidrule(lr){3-8} \cmidrule(lr){9-14}
    Method   &  & 3 & 5 & 10 & 30 & 45 & $\eta$ & 0.05 & 0.1 & 0.25 & 0.5 & 0.75 & $\eta$ \\\midrule
    \multirow{4}{*}{EIG-SE3} 
    & Vanilla  &    
         \begin{tabular}[c]{@{}c@{}}11.99\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}23.87\\{\tiny$\pm$0.00}\end{tabular}   &  
         \begin{tabular}[c]{@{}c@{}}34.49\\{\tiny$\pm$0.00}\end{tabular}   & 
         \begin{tabular}[c]{@{}c@{}}57.59\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}62.09\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}}25.37\\{\tiny$\pm$0.00}\end{tabular}  &
         
         \begin{tabular}[c]{@{}c@{}} 0.00\\{\tiny$\pm$0.00}\end{tabular}   & 
         \begin{tabular}[c]{@{}c@{}} 0.06\\{\tiny$\pm$0.00}\end{tabular}   &   
         \begin{tabular}[c]{@{}c@{}} 2.63\\{\tiny$\pm$0.00}\end{tabular}   & 
         \begin{tabular}[c]{@{}c@{}}31.39\\{\tiny$\pm$0.00}\end{tabular}   &  
         \begin{tabular}[c]{@{}c@{}}74.40\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}} 0.61\\{\tiny$\pm$0.00}\end{tabular} \\
         \cmidrule(lr){3-14} 
     & w. PoserNet     &  
         \begin{tabular}[c]{@{}c@{}}15.56\\ {\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}48.36\\{\tiny$\pm$0.00}\end{tabular}   &  
         \begin{tabular}[c]{@{}c@{}}82.14\\{\tiny$\pm$0.00}\end{tabular}   & 
         \begin{tabular}[c]{@{}c@{}}93.14\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}95.69\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}} 5.10\\{\tiny$\pm$0.00}\end{tabular}  &

         \begin{tabular}[c]{@{}c@{}} 0.04\\{\tiny$\pm$0.00}\end{tabular}   & 
         \begin{tabular}[c]{@{}c@{}} 1.94\\{\tiny$\pm$0.00}\end{tabular}   &   
         \begin{tabular}[c]{@{}c@{}}34.51\\{\tiny$\pm$0.00}\end{tabular}   & 
         \begin{tabular}[c]{@{}c@{}}76.43\\{\tiny$\pm$0.00}\end{tabular}   &  
         \begin{tabular}[c]{@{}c@{}}94.49\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}}0.32\\{\tiny$\pm$0.00}\end{tabular} \\
     & w. PoserNet v2     &  
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}   &  
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}   & 
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  &
         
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}   & 
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}   &   
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}   & 
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}   &  
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}
         
    \\\midrule
    \multirow{6}{*}{RAGO} & Vanilla      & 
         \begin{tabular}[c]{@{}c@{}}20.95\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}47.20\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}73.51\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}93.05\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}96.27\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}} 5.32\\{\tiny$\pm$0.00}\end{tabular}  &
         
         \begin{tabular}[c]{@{}c@{}} 0.13\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}} 1.01\\{\tiny$\pm$0.00}\end{tabular}  &   
         \begin{tabular}[c]{@{}c@{}} 7.44\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}35.75\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}69.68\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}} 0.60\\{\tiny$\pm$0.00}\end{tabular}    \\  \cmidrule(lr){3-14}
         
         & w. PoserNet v2      & 
         \begin{tabular}[c]{@{}c@{}}27.11\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}57.41\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}84.40\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}95.96\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}97.59\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}} 4.41\\{\tiny$\pm$0.00}\end{tabular}  &
         
         \begin{tabular}[c]{@{}c@{}}1.50\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}11.59\\{\tiny$\pm$0.00}\end{tabular}  &   
         \begin{tabular}[c]{@{}c@{}}40.97\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}71.58\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}90.09\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}}0.31\\{\tiny$\pm$0.00}\end{tabular}    \\  \cmidrule(lr){3-14}

        & Joint (simple loss sum) & 
         \begin{tabular}[c]{@{}c@{}}35.92\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}63.02\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}86.29\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}96.24\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}97.56\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}}3.92\\{\tiny$\pm$0.00}\end{tabular}  &
         
         \begin{tabular}[c]{@{}c@{}} 0.34\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}} 4.47\\{\tiny$\pm$0.00}\end{tabular}  &   
         \begin{tabular}[c]{@{}c@{}}33.23\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}67.84\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}89.41\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}} 0.36\\{\tiny$\pm$0.00}\end{tabular}    \\  
         
         \midrule
    \multirow{4}{*}{NeuRoRA} & Vanilla      & 
         \begin{tabular}[c]{@{}c@{}}16.03\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}41.03\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}69.35\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}91.35\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}95.96\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}} 6.04\\{\tiny$\pm$0.00}\end{tabular}  &
         
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  &   
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}    \\  \cmidrule(lr){3-14}

         & w. PoserNet v2     & 
         \begin{tabular}[c]{@{}c@{}}21.44\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}53.99\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}83.91\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}95.97\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}97.39\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}} 4.71\\{\tiny$\pm$0.00}\end{tabular}  &
         
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  &   
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  & 
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  &  
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}  &       
         \begin{tabular}[c]{@{}c@{}}0.00\\{\tiny$\pm$0.00}\end{tabular}    \\ 
    \bottomrule
    \end{tabularx}
    \centering
    \caption{\label{tab:results_posernet_bb_vs_keypoints}
    Absolute pose error. Note: Say we skip graphs with more than one component because our graphs are already quite small (we keep 6731 graphs out of 7000). All results are expressed as medians of graph-wise means. Histograms are computed based on single-node errors, so we have $n\_graphs \times 8$ errors. Results for EIG-SE3 have been copied from the ECCV paper, so no graphs have been filtered out. Vanilla NeuRoRA performs quite a lot better than vanilla EIG-SE3. This probably happens because vanilla NeuRoRA is actually fine-tuned on our 5pts training data.}
    % describes data used as input for PoserNet, while ``Refined'' describes its output. $\eta$ indicates median values. For both initialisation techniques, Both for BB and keypoint based input, PoserNet is effective at refining relative poses in terms of orientation and translation direction.}


\end{table*}

\begin{figure*}[th!]
        \centering
    \begin{tabular}{|c|c|c|}
          \hline
          \includegraphics[width=55mm]{Images/with_vs_without_PN_NeuRoRA_logY_transparent.pdf} & \includegraphics[width=55mm]{Images/with_vs_without_PN_RAGO_logY_transparent.pdf}    &
          \includegraphics[width=55mm]{Images/joint_PN_and_RAGO_logY_transparent.pdf}          \\
          
          \includegraphics[width=55mm]{Images/with_vs_without_PN_NeuRoRA_transparent.pdf}      & \includegraphics[width=55mm]{Images/with_vs_without_PN_RAGO_transparent.pdf}         &
          \includegraphics[width=55mm]{Images/joint_PN_and_RAGO_transparent.pdf}               \\
          
          \small NeuRoRA &  RAGO & Joint PN, RAGO\\
          \hline
    \end{tabular}
    \caption{ Temp figure so that we can look at the histograms all together.
    %\emph{Effect of PoserNet+ refinement on downstream tasks}: error distribution for all camera absolute orientations generated by NeuRoRa~\cite{purkait2020neurora} (a) and RAGO~\cite{li2022rago} (c) with (yellow) and without (blue) PoserNet refinement. For ease of viewing, we present the same distributions in semi-log scale (b,d respectively).%
    }\label{fig:temp_figure}
\end{figure*}

\begin{figure*}
        \centering
    \begin{tabular}{|c|}
          \hline
          \includegraphics[width=55mm]{Images/joint_vs_separated_PN_and_RAGO_logY_transparent.pdf} \\  
          \includegraphics[width=55mm]{Images/joint_vs_separated_PN_and_RAGO_transparent.pdf}      \\ 
          \hline
    \end{tabular}
    \caption{ Effect of training PN and RAGO separately or joint.}\label
    {fig:temp_figure}
\end{figure*}

